Ramsey numbers of trees

We show that there exists a constant $c>0$ such that every $n$-vertex tree $T$ with $\Delta(T)\le cn$ has Ramsey number $R(T)=\max\{t_1+2t_2,2t_1\}-1$, where $t_1\ge t_2$ are the sizes of the bipartition classes of $T$. This improves an asymptotic result of Haxell, {\L}uczak, and Tingley from 2002, and shows that, though Burr's 1974 conjecture on the Ramsey numbers of trees has long been known to be false for certain `double stars', it is true for trees with up to small linear maximum degree.

==> figures/ClaimA/ClaimA-1.tex <==
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.25*\ver)$);

\draw[red,fill=red!60] ($(B)+(0.6,0)$) -- ($(B)+(0.5,0)$) -- ($(C)+(0.5,0)$) -- ($(C)+(0.6,0)$) -- cycle;

\draw[red,fill=red!60] ($(A)+(0,0.6)$) -- ($(A)-(0,0.6)$) -- ($(B)-(0,0.6)$) -- ($(B)+(0,0.6)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[fill=white] (A) circle [radius=0.6cm];
\draw[fill=white] (B) circle [radius=0.6cm];
\draw[fill=white] (C) circle [radius=0.6cm];

\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw (C) node {$I_C$};


\draw ($(A)+(-0.8,0.5)$) node {$t_1^-$};
\draw ($(B)+(0.9,0.5)$) node {$t_2^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$t_2^-$};

\end{tikzpicture}


==> figures/ClaimA/ClaimA-2.tex <==
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.25*\ver)$);

\draw[red,fill=red!60] ($(B)+(0.6,0)$) -- ($(B)+(0.5,0)$) -- ($(C)+(0.5,0)$) -- ($(C)+(0.6,0)$) -- cycle;

\draw[red,fill=red!60] ($(A)+(0,0.6)$) -- ($(A)-(0,0.6)$) -- ($(B)-(0,0.6)$) -- ($(B)+(0,0.6)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[white,fill=white] ($(A)-(0.6,0)$) -- ($(C)-(0.6,0)$) -- ($(C)+(0.6,0)$) -- ($(A)+(0.6,0)$) -- cycle;
\draw[blue,pattern=crosshatch, pattern color=blue!50] ($(A)-(0.6,0)$) -- ($(C)-(0.6,0)$) -- ($(C)+(0.6,0)$) -- ($(A)+(0.6,0)$) -- cycle;


\draw[fill=white] (A) circle [radius=0.6cm];
\draw[fill=white] (B) circle [radius=0.6cm];
\draw[fill=white] (C) circle [radius=0.6cm];

\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw (C) node {$I_C$};


\draw ($(A)+(-0.8,0.5)$) node {$t_1^-$};
\draw ($(B)+(0.9,0.5)$) node {$t_2^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$t_2^-$};

\end{tikzpicture}


==> figures/ClaimA/ClaimA-3.tex <==
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.25*\ver)$);

\draw[red,fill=red!60] ($(B)+(0.6,0)$) -- ($(B)+(0.5,0)$) -- ($(C)+(0.5,0)$) -- ($(C)+(0.6,0)$) -- cycle;

\draw[red,fill=red!60] ($(A)+(0,0.6)$) -- ($(A)-(0,0.6)$) -- ($(B)-(0,0.6)$) -- ($(B)+(0,0.6)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[white,fill=white] ($(A)-(0.6,0)$) -- ($(C)-(0.6,0)$) -- ($(C)+(0.6,0)$) -- ($(A)+(0.6,0)$) -- cycle;
\draw[blue,pattern=crosshatch, pattern color=blue!50] ($(A)-(0.6,0)$) -- ($(C)-(0.6,0)$) -- ($(C)+(0.6,0)$) -- ($(A)+(0.6,0)$) -- cycle;

\draw[white,fill=white] ($(B)+(0.4,0)$) -- ($(B)+(0.3,0)$) -- ($(C)+(0.3,0)$) -- ($(C)+(0.4,0)$) -- cycle;
\draw[blue,pattern=crosshatch, pattern color=blue!50] ($(B)+(0.4,0)$) -- ($(B)+(0.3,0)$) -- ($(C)+(0.3,0)$) -- ($(C)+(0.4,0)$) -- cycle;

\draw[fill=white] (A) circle [radius=0.6cm];
\draw[fill=white] (B) circle [radius=0.6cm];
\draw[fill=white] (C) circle [radius=0.6cm];

\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw (C) node {$I_C$};


\draw ($(A)+(-0.8,0.5)$) node {$t_1^-$};
\draw ($(B)+(0.9,0.5)$) node {$t_2^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$t_2^-$};

\end{tikzpicture}


==> figures/ClaimA/ClaimA-4.tex <==
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.25*\ver)$);
\coordinate (V) at ($0.5*(A)+0.5*(C)$) {};


\draw[red,fill=red!60] ($(B)+(0.6,0)$) -- ($(B)+(0.5,0)$) -- ($(C)+(0.5,0)$) -- ($(C)+(0.6,0)$) -- cycle;

\draw[red,fill=red!60] ($(A)+(0,0.6)$) -- ($(A)-(0,0.6)$) -- ($(B)-(0,0.6)$) -- ($(B)+(0,0.6)$) -- cycle;

\draw[red,fill=red!60] ($(A)+(0,0.08)$) -- ($(A)-(0,0.08)$) -- ($(V)-(0,0.08)$) -- ($(V)+(0,0.08)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;



\draw[fill=white] (A) circle [radius=0.6cm];
\draw[fill=white] (B) circle [radius=0.6cm];
\draw[fill=white] (C) circle [radius=0.6cm];

\draw[->,thick] ($(A)+(-0.1,0.1)-(0.3,0.4)+(0.06,-0.04)-(-0.05,0.05)-(0.05,0)$) to[out=-70,in=180]  ($(V)-(0.15,0)$);

\draw[fill=white] (V) circle [radius=0.1cm];

\draw[red,fill=red!60] ($(A)+(-0.1,0.1)-(0.3,0.4)$) --++ (0.6,0) --++ (0,-0.08) --++ (-0.6,0) -- cycle;

\draw[fill=white] ($(A)+(-0.1,0.1)-(0.3,0.4)+(0.06,-0.04)$) circle [radius=0.1cm];

% ($(A)-(0,0.6)$) -- ($(B)-(0,0.6)$) -- ($(B)+(0,0.6)$) -- cycle;


\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw (C) node {$I_C$};



%\node[main] (V0) at (V) {};


\draw ($(A)+(-0.8,0.5)$) node {$t_1^-$};
\draw ($(B)+(0.9,0.5)$) node {$t_2^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$t_2^-$};

\end{tikzpicture}


==> figures/ClaimB/ClaimB-1.tex <==
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.25*\ver)$);

\draw[red,fill=red!60] ($(A)-(0.6,0)$) -- ($(A)-(0.5,0)$) -- ($(C)-(0.5,0)$) -- ($(C)-(0.6,0)$) -- cycle;

\draw[red,fill=red!60] ($(A)+(0,0.6)$) -- ($(A)-(0,0.6)$) -- ($(B)-(0,0.6)$) -- ($(B)+(0,0.6)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[fill=white] (A) circle [radius=0.6cm];
\draw[fill=white] (B) circle [radius=0.6cm];
\draw[fill=white] (C) circle [radius=0.6cm];

\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw (C) node {$I_C$};


\draw ($0.5*(A)+0.5*(B)+(0,1)$) node {$n^-$};
\draw ($(A)+(-1.1,0.5)$) node {$\geq t_2^+$};
\draw ($(B)+(1.1,0.5)$) node {$\geq t_2^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(1,0)$) node {$t_2^-$};

\end{tikzpicture}


==> figures/ClaimB/ClaimB-2.tex <==
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.25*\ver)$);

\draw[red,fill=red!60] ($(A)-(0.6,0)$) -- ($(A)-(0.5,0)$) -- ($(C)-(0.5,0)$) -- ($(C)-(0.6,0)$) -- cycle;

\draw[red,fill=red!60] ($(A)+(0,0.6)$) -- ($(A)-(0,0.6)$) -- ($(B)-(0,0.6)$) -- ($(B)+(0,0.6)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;

\draw[white,fill=white] (A) circle [radius=0.6cm];
\draw[white,fill=white] (B) circle [radius=0.6cm];

\draw[blue,pattern=crosshatch, pattern color=blue!50] (A) circle [radius=0.6cm];
\draw[blue,pattern=crosshatch, pattern color=blue!50] (B) circle [radius=0.6cm];
\draw[fill=white] (C) circle [radius=0.6cm];

\draw[white,fill=white] (A) circle [radius=0.3cm];
\draw[white,fill=white] (B) circle [radius=0.3cm];
%\draw[white,line width=0pt,pattern=crosshatch, pattern color=blue!20] (A) circle [radius=0.3cm];
%\draw[white,ultra thin,pattern=crosshatch, pattern color=blue!20] (B) circle [radius=0.3cm];

\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw (C) node {$I_C$};


\draw ($0.5*(A)+0.5*(B)+(0,1)$) node {$n^-$};
\draw ($(A)+(-1.1,0.5)$) node {$\geq t_2^+$};
\draw ($(B)+(1.1,0.5)$) node {$\geq t_2^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(1,0)$) node {$t_2^-$};

\end{tikzpicture}


==> figures/ClaimB/ClaimB-3.tex <==
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.25*\ver)$);
\coordinate (A0) at ($(A)+(0,-\Ahgt-2.25*\ver+0.45)$);
\coordinate (B0) at ($(B)+(0,-\Ahgt-2.25*\ver+0.45)$);

\draw[white] (0,0) -- (0,-2.5);


\draw[red,fill=red!60] ($(A)+(0,0.6)$) -- ($(A)-(0,0.6)$) -- ($(B)-(0,0.6)$) -- ($(B)+(0,0.6)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;

\draw[red,fill=red!60] ($(A)-(0.6,0)$) -- ($(A)+(0.6,0)$) -- ($(B0)+(0,0.4)$) -- ($(B0)-(0,0.4)$) -- cycle;
\draw[red,fill=red!60] ($(B)-(0.6,0)$) -- ($(B)+(0.6,0)$) -- ($(A0)+(0.4,0)$) -- ($(A0)+(0,0.4)$) -- cycle;


\draw[white,fill=white] (A) circle [radius=0.6cm];
\draw[white,fill=white] (B) circle [radius=0.6cm];

\draw[blue,pattern=crosshatch, pattern color=blue!50] (A) circle [radius=0.6cm];
\draw[blue,pattern=crosshatch, pattern color=blue!50] (B) circle [radius=0.6cm];
\draw[fill=white] (A0) circle [radius=0.4cm];
\draw[fill=white] (B0) circle [radius=0.4cm];

\draw[white,fill=white] (A) circle [radius=0.3cm];
\draw[white,fill=white] (B) circle [radius=0.3cm];
%\draw[white,line width=0pt,pattern=crosshatch, pattern color=blue!20] (A) circle [radius=0.3cm];
%\draw[white,ultra thin,pattern=crosshatch, pattern color=blue!20] (B) circle [radius=0.3cm];

\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw ($(A0)$) node {$I_A'$};
\draw ($(B0)$) node {$I_B'$};


\draw ($0.5*(A)+0.5*(B)+(0,1)$) node {$n^-$};
\draw ($(A)+(-1.1,0.5)$) node {$\geq t_2^+$};
\draw ($(B)+(1.1,0.5)$) node {$\geq t_2^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};

\end{tikzpicture}


==> figures/ClaimB/ClaimB-4.tex <==
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.25*\ver)$);
\coordinate (A0) at ($(A)+(0,-\Ahgt-2.25*\ver+0.45)$);
\coordinate (B0) at ($(B)+(0,-\Ahgt-2.25*\ver+0.45)$);


\draw[white] (0,0) -- (0,-2.5);



\draw[red,fill=red!60] ($(A)+(0,0.6)$) -- ($(A)-(0,0.6)$) -- ($(B)-(0,0.6)$) -- ($(B)+(0,0.6)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;

\draw[red,fill=red!60] ($(A)-(0.6,0)$) -- ($(A)+(0.6,0)$) -- ($(B0)+(0,0.4)$) -- ($(B0)-(0,0.4)$) -- cycle;
\draw[red,fill=red!60] ($(B)-(0.6,0)$) -- ($(B)+(0.6,0)$) -- ($(A0)+(0.4,0)$) -- ($(A0)+(0,0.4)$) -- cycle;


\draw[white,fill=white] ($(A)-(0.6,0)$) arc (180:0:0.6) -- ($(A0)+(0.4,0)$) arc (0:-180:0.4) -- cycle;
\draw[white,fill=white] ($(B)-(0.6,0)$) arc (180:0:0.6) -- ($(B0)+(0.4,0)$) arc (0:-180:0.4) -- cycle;

\draw[blue,pattern=crosshatch, pattern color=blue!50] ($(A)-(0.6,0)$) arc (180:0:0.6) -- ($(A0)+(0.4,0)$) arc (0:-180:0.4) -- cycle;
\draw[blue,pattern=crosshatch, pattern color=blue!50] ($(B)-(0.6,0)$) arc (180:0:0.6) -- ($(B0)+(0.4,0)$) arc (0:-180:0.4) -- cycle;

%\draw[blue,pattern=crosshatch, pattern color=blue!50] (A) circle [radius=0.6cm];
%\draw[blue,pattern=crosshatch, pattern color=blue!50] (B) circle [radius=0.6cm];


\draw[white,fill=white] (A) circle [radius=0.3cm];
\draw[white,fill=white] (B) circle [radius=0.3cm];
\draw[white,fill=white] ($(A0)+(0,0.2)$) circle [radius=0.35cm];
\draw[white,fill=white] ($(B0)+(0,0.2)$) circle [radius=0.35cm];
%\draw[white,line width=0pt,pattern=crosshatch, pattern color=blue!20] (A) circle [radius=0.3cm];
%\draw[white,ultra thin,pattern=crosshatch, pattern color=blue!20] (B) circle [radius=0.3cm];

\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw ($(A0)+(0,0.2)$) node {$I_A'$};
\draw ($(B0)+(0,0.2)$) node {$I_B'$};


\draw ($0.5*(A)+0.5*(B)+(0,1)$) node {$(n+t_2)^-$};
\draw ($(A)+(-1.1,0.5)$) node {$\geq t_2^+$};
\draw ($(B)+(1.1,0.5)$) node {$\geq t_2^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};

\end{tikzpicture}


==> figures/EM1a/aEM1a-1.tex <==
\begin{center}
\begin{tikzpicture}[scale=0.7,main1/.style = {circle,draw,fill=none,inner sep=2}, main2/.style = {circle,draw,fill=none,inner sep=3}, main3/.style = {circle,draw,fill=none,inner sep=1.5}]


\node[main1] (A0) at (0.5,0) {};
\node[main1] (A1) at (2,1) {};
\node[main1] (A2) at (2,0.5) {};
\node[main1] (A3) at (2,0) {};
%\node[draw=none,fill=none] at (2,-0.4) {$\vdots$};

\node[main2] (C1) at (0.5,2) {};
\node[main2] (C2) at (0.5,1.5) {};
\node[main2] (C3) at (0.5,1) {};


\node[main2] (B1) at (3.25,1) {};
\node[main2] (B2) at (3.25,0.5) {};

\node[main2] (B3) at (3.25,0) {};
%\node[draw=none,fill=none] at (3.5,-0.4) {$\vdots$};


\node[main1] (J0) at ($(B1)+(0,1.5)$) {};
\node[main1] (I1) at ($(B2)+(2.5,0)$) {};



\coordinate (A4) at (2,-1) {};
%\coordinate (A5) at (2,-1) {};


\def\spr{0.4};

\foreach \y in {1,2,3}
{
\node[main1] (D\y) at ($(B\y)+(1.25,0)$) {};
\draw[red,thick] (A\y) -- (C\y);
}

\foreach \y in {2,3}
{
\draw[red,thick] (I1) -- (D\y);
}


\draw[red,thick] (A0) to[out=75,in=180] (J0);
\draw[red,thick] (J0) to[out=0,in=125] (I1);



\coordinate (B4) at (3.7,-1) {};
\coordinate (B5) at (3.7,-1.8) {};
\draw[red,thick] (B4) -- (B5);
\draw[red,thick] (A0) to[out=-20,in=180] (B4);
\draw[red,thick] (A0) to[out=-45,in=180] (B5);
\draw ($0.25*(A3)+0.25*(B3)+0.25*(A4)+0.25*(B4)-(-0.18,0.7)$) node {\textbf{H\L T$^-$}};



\foreach \x/\y in {1/1,2/2,3/3}
{
\draw[red,thick] (B\x) -- (D\y);
}

\foreach \n in {1,2,3}
{
\draw[red,thick] (A0) -- (A\n);
}

\foreach \n in {1}
{
\draw[red,thick] (A\n) -- (B\n);
}

\draw[red,thick] (A1) -- (C1);
\draw[red,thick] (A2) -- (C2);

%\draw ($0.5*(A1)+0.5*(C1)+(0,0.4)$) node {$M'$};
%\draw ($(A4)-(0,0.5)$) node {$t_2^-$};
%\draw ($(B4)-(0,0.55)$) node {$t_1^+$};



\draw ($(A0)-(0.4,0)$) node {$i_1$};
\draw ($(J0)-(-0.2,0.4)$) node {$i_2$};
\draw ($(I1)+(0.4,0)$) node {$i_3$};


\draw ($(A1)+(0,0.55)$) node {$I_{0/1,1}$};
\draw ($(C1)+(0,0.6)$) node {$I_{1,2}$};
\draw ($(A1)+(0,-3.15)$) node {$I_{1,1}$};
\draw ($(B1)+(0,-3.15)$) node {$I_{1,2}$};
\draw ($(B1)+(0,0.5)$) node {$I_{0,2}$};
\draw ($(D1)+(0,0.5)$) node {$I_{0,3}$};
\draw ($(B1)+(0,-1.5)$) node {$I_{3,2}$};
\draw ($(D1)+(0,-1.5)$) node {$I_{3,1}$};
\end{tikzpicture}
\end{center}

==> figures/EM1a/aEM1a-2.tex <==
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=none,inner sep=1.5}, main2/.style = {circle,draw,fill=none,inner sep=2.25}]
\def\spacer{1.25};
\def\spacerr{1.25};
\def\Ahgt{1.2};
\def\Bhgt{1.2};

%\draw [fill=white,white] (0,1.35) circle [x radius=0.6cm,y radius=0.75cm];
%\draw [fill=white,white] (0,-1.45) circle [x radius=0.6cm,y radius=0.7cm];


\coordinate (B) at (\spacer,0);


\node[main1] (V1) at ($(-\spacerr,1.35)$) {};
\node[main1] (V2) at ($(-\spacerr,-0.1)$) {};
\node[main1] (V3) at ($(-\spacerr,-1.45)$) {};

\node[main1] (A1) at (0,1.35) {};
%\node[main1] (A2) at (0,-0.1) {};
\node[main1] (A3) at (0,-1.45) {};
\foreach \n in {1,3}
{
\node[main1] (B\n) at ($(A\n)+(\spacer,0)$) {};
}

\node[main1] (A0) at ($(A1)+(0,1.35)$) {};
\node[main1] (B0) at ($(B1)+(0,1.35)$) {};
\node[main1] (C0) at ($(B0)+(\spacer,0)$) {};
\draw [thick,red] (V1) -- (A0) -- (B0) -- (C0);

\foreach \n in {1,3}
{
\draw [thick,red] (V\n) -- (A\n) -- (B\n);
}

\draw [thick,red] (V1) -- (V2) -- (V3);

\draw ($(V1)-(0.5,0)$) node {$i_1$};
\draw ($(V2)-(0.5,0)$) node {$i_2$};
\draw ($(V3)-(0.5,0)$) node {$i_3$};
\foreach \where/\what in {A1/I_{1,1},B1/I_{1,2},A3/I_{3,1},B3/I_{3,2},A0/I_{0,1},B0/I_{0,2},C0/I_{0,3}}
{
\draw ($(\where)+(-0.1,0.5)$) node {$\what$};
}


\draw ($(-\spacerr,0.625)-(1.8,0)$) node {$R_{\text{\bfseries EM1a}}':$};





%\draw (10.5,2) node {Type II};
\end{tikzpicture}


==> figures/EM1a/aEM1a.tex <==
\begin{center}
\begin{tikzpicture}[scale=0.7,main1/.style = {circle,draw,fill=none,inner sep=2}, main2/.style = {circle,draw,fill=none,inner sep=3}, main3/.style = {circle,draw,fill=none,inner sep=1.5}]


\node[main1] (A0) at (0.5,0) {};
\node[main1] (A1) at (2,1) {};
\node[main1] (A2) at (2,0.5) {};
\node[main1] (A3) at (2,0) {};
%\node[draw=none,fill=none] at (2,-0.4) {$\vdots$};

\node[main2] (C1) at (0.5,2) {};
\node[main2] (C2) at (0.5,1.5) {};
\node[main2] (C3) at (0.5,1) {};


\node[main2] (B1) at (3.25,1) {};
\node[main2] (B2) at (3.25,0.5) {};
\node[main2] (B3) at (3.25,0) {};
%\node[draw=none,fill=none] at (3.5,-0.4) {$\vdots$};



\coordinate (A4) at (2,-1) {};
%\coordinate (A5) at (2,-1) {};


\def\spr{0.4};

\foreach \y in {1,...,6}
{
\node[main1] (D\y) at ($(4.5,1.9-\y*\spr)$) {};
}



\foreach \x in {1,2,3}
\draw[red,thick] (A\x) -- (C\x);

\coordinate (B4) at (3.7,-0.5) {};
\coordinate (B5) at (3.7,-1.3) {};
\draw[red,thick] (B4) -- (B5);
\draw[red,thick] (A0) to[out=-20,in=180] (B4);
\draw[red,thick] (A0) to[out=-45,in=180] (B5);
\draw ($0.25*(A3)+0.25*(B3)+0.25*(A4)+0.25*(B4)-(-0.1,0.4)$) node {\textbf{H\L T$^-$}};

\draw ($0.5*(A1)+0.5*(B1)+(0,2)$) node {$R_{\text{\bfseries EM1a}}:$};

\foreach \x/\y in {1/1,1/3,1/5,2/2,2/6,3/5,3/2,3/4}
{
\draw[red,thick] (B\x) -- (D\y);
}

\foreach \n in {1,2,3}
{
\draw[red,thick] (A\n) -- (B\n);
\draw[red,thick] (A0) -- (A\n);
}

\draw[red,thick] (A1) -- (C1);
\draw[red,thick] (A2) -- (C2);

%\draw ($0.5*(A1)+0.5*(C1)+(0,0.4)$) node {$M'$};
%\draw ($(A4)-(0,0.5)$) node {$t_2^-$};
%\draw ($(B4)-(0,0.55)$) node {$t_1^+$};



\draw ($(A0)-(0.4,0)$) node {$0$};

\draw ($(A1)+(0,0.55)$) node {$I_A'$};
\draw ($(C1)+(0,0.6)$) node {$I_B''$};
\draw ($(B1)+(0,0.55)$) node {$I_B'$};
\draw ($(D1)+(0,0.5)$) node {$I_C$};
\draw ($(A1)+(0,-2.75)$) node {$I_A$};
\draw ($(B1)+(0,-2.75)$) node {$I_B$};


%\draw ($(D23)+(0.1,0)-(0,0.5)$) node {$0^+$};
\draw ($(A1)+(0,-2.65)$) node {$\phantom{I_{1,1}}$};
\draw ($(B1)+(0,-2.65)$) node {$\phantom{I_{1,2}}$};
\end{tikzpicture}
\end{center}



==> figures/EM2a/aEM2a-1.tex <==
\begin{center}
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=none,inner sep=1.2},main2/.style = {circle,draw,fill=none,inner sep=0.8}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0,-\Ahgt-2.5*\ver)$);


\draw[red,fill=red!20] ($(A)+(0,\Ahgt)$) -- ($(A)-(0,\Ahgt)$) -- ($(B)-(0,\Bhgt)$) -- ($(B)+(0,\Bhgt)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[fill=white,densely dotted] (A) circle [y radius=\Ahgt cm,x radius=0.6cm];
\draw[fill=white,densely dotted] (B) circle [y radius=\Bhgt cm,x radius=0.6cm];
\draw[fill=white,densely dotted] (C) circle [y radius=0.35 cm,x radius=0.35cm];

%\draw ($(A)+(0,0.5*\Ahgt)-(0.5,0)$) node {$I_A$};
%\draw ($(B)+(0.5,0)$) node {$I_B$};
%\draw ($(C)+(0,0.5)$) node {$I_C$};


\draw ($(A)+(-1,0)-(0.2,-0.2)$) node {$\geq t_2^+$};
\draw ($(B)+(1,0)+(0.2,-0.2)$) node {$\geq t_2^-$};
\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$0^+$};

\node[main1] (i) at ($(A)+(-0.1,0.3)$) {};
\node[main1] (j) at ($(i)-(0,0.5*\Ahgt)+(0.1,-0.15)$) {};
\node[main1] (A3) at ($(i)-(0,0.8*\Ahgt)+(-0.02,0.02)-(0,0.27)$) {};
\node[main1] (A4) at ($(A3)-(0.15,-0.13)$) {};
\node[main1] (A5) at ($(A3)+(0.15,-0.13)$) {};
\node[main2] (B3) at (C) {};
\node[main2] (B4) at ($(B3)-(0.2,0)$) {};
\node[main2] (B5) at ($(B3)+(0.2,0)$) {};

\node [main1] (D1) at ($(A)+(0.3,0)$) {};
\node [main1] (D2) at ($(A)+(0.2,-0.15)$) {};
\node [main1] (D3) at ($(A)+(0.4,0.15)$) {};
\node [main2] (E1) at ($(B)+(0,-0.2)+(0,0)$) {};
\node [main2] (E2) at ($(B)+(0,-0.2)+(0,-0.15)$) {};
\node [main2] (E3) at ($(B)+(0,-0.2)+(0,0.15)$) {};

\node [main2] (F1) at ($(A)+(0,0.7)+(0,0)$) {};
\node [main2] (F2) at ($(A)+(0,0.7)+(0,-0.15)$) {};
\node [main2] (F3) at ($(A)+(0,0.7)+(0,0.15)$) {};
\node [main1] (G1) at ($(B)+(0,0.6)+(0,0)$) {};
\node [main1] (G2) at ($(B)+(0,0.6)+(0,-0.2)$) {};
\node [main1] (G3) at ($(B)+(0,0.6)+(0,0.2)$) {};

\foreach \n in {1,2,3}
{
\draw [red,thick] (j) -- (E\n) -- (D\n);
\draw [red,thick] (i) -- (G\n) -- (F\n);
}


\node[main1] (ipr) at ($(B)-(0,0.8*\Ahgt)$) {};

\draw [red,thick] (j) -- (ipr);
\foreach \n in {3,4,5}
{
\draw[red,thick] (ipr) -- (A\n) -- (B\n);
}

\draw[red,thick] (i) -- (j);


\draw ($(i)+(-0.225,0.1)$) node {\footnotesize $i_1$};
\draw ($(j)+(-0.25,0.1)$) node {\footnotesize $i_2$};
\draw ($(ipr)+(0.275,0.15)$) node {\footnotesize $i_3$};

\end{tikzpicture}
\end{center}


==> figures/EM2a/aEM2a-2.tex <==
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=none,inner sep=1.5}, main2/.style = {circle,draw,fill=none,inner sep=2.25}]
\def\spacer{2};
\def\spacerr{1.5};
\def\Ahgt{1.2};
\def\Bhgt{1.2};

\draw [fill=white,white] (0,1.35) circle [x radius=0.6cm,y radius=0.75cm];
\draw [fill=white,white] (0,-1.45) circle [x radius=0.6cm,y radius=0.7cm];


\coordinate (B) at (\spacer,0);


\node[main1] (V1) at ($(-\spacerr,1.35)$) {};
\node[main1] (V2) at ($(-\spacerr,-0.1)$) {};
\node[main1] (V3) at ($(-\spacerr,-1.45)$) {};

\node[main1] (A1) at (0,1.35) {};
\node[main1] (A2) at (0,-0.1) {};
\node[main1] (A3) at (0,-1.45) {};
\foreach \n in {1,2,3}
{
\node[main1] (B\n) at ($(A\n)+(\spacer,0)$) {};
}



\foreach \n in {1,2,3}
{
\draw [thick,red] (V\n) -- (A\n) -- (B\n);
}

\draw [thick,red] (V1) -- (V2) -- (V3);

\draw ($(V1)-(0.5,0)$) node {$i_1$};
\draw ($(V2)-(0.5,0)$) node {$i_2$};
\draw ($(V3)-(0.5,0)$) node {$i_3$};
\foreach \where/\what in {A1/I_{1,1},B1/I_{1,2},A2/I_{2,1},B2/I_{2,2},A3/I_{3,1},B3/I_{3,2}}
{
\draw ($(\where)+(0,0.5)$) node {$\what$};
}


\draw ($(V2)-(1.8,0)$) node {$R_{\text{\bfseries EM2a}}':$};





%\draw (10.5,2) node {Type II};
\end{tikzpicture}


==> figures/EM2a/aEM2a.tex <==
\begin{center}
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0,-\Ahgt-2.5*\ver)$);

\draw[red,thick] ($(A)-(0.3,0)$) -- ($(C)-(0.3,0)$);
\draw[red,thick] ($(A)-(0.1,0)$) -- ($(C)-(0.1,0)$);
\draw[red,thick] ($(A)-(-0.1,0)$) -- ($(C)-(-0.1,0)$);
\draw[red,thick] ($(A)-(-0.3,0)$) -- ($(C)-(-0.3,0)$);

\draw[red,fill=red!60] ($(A)+(0,\Ahgt)$) -- ($(A)-(0,\Ahgt)$) -- ($(B)-(0,\Bhgt)$) -- ($(B)+(0,\Bhgt)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[fill=white] (A) circle [y radius=\Ahgt cm,x radius=0.6cm];
\draw[fill=white] (B) circle [y radius=\Bhgt cm,x radius=0.6cm];
\draw[fill=white] (C) circle [y radius=0.35 cm,x radius=0.35cm];

\draw ($(A)+(0,0.5*\Ahgt)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw (C) node {$I_C$};
\draw ($(C)+(-1,0.85)$) node {$M$};

\draw ($(A)+(-0.75,1.75)$) node {$R_{\text{{\bfseries EM2a}}}:$};

\draw ($(A)+(-1,0)-(0.2,-0.2)$) node {$\geq t_2^+$};
\draw ($(B)+(1,0)+(0.2,-0.2)$) node {$\geq t_2^-$};
\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$0^+$};

\node[main] (A1) at (A) {};
\node[main] (A2) at ($(A)-(0,0.5*\Ahgt)$) {};

\draw[red,thick] (A1) -- (A2);
\end{tikzpicture}
\end{center}


==> figures/EM2b/aEM2b-1.tex <==
\begin{center}
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=none,inner sep=1.2},main2/.style = {circle,draw,fill=none,inner sep=0.8}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0,-\Ahgt-2.5*\ver)$);


\draw[red,fill=red!20] ($(A)+(0,\Ahgt)$) -- ($(A)-(0,\Ahgt)$) -- ($(B)-(0,\Bhgt)$) -- ($(B)+(0,\Bhgt)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[fill=white,densely dotted] (A) circle [y radius=\Ahgt cm,x radius=0.6cm];
\draw[fill=white,densely dotted] (B) circle [y radius=\Bhgt cm,x radius=0.6cm];
\draw[fill=white,densely dotted] (C) circle [y radius=0.35 cm,x radius=0.35cm];



\draw ($(A)+(-1,0)-(0.2,-0.2)$) node {$\geq t_2^+$};
\draw ($(B)+(1,0)+(0.2,-0.2)$) node {$\geq t_2^-$};
%\draw ($(A)+(-1,0)$) node {$t_2^+$};
%\draw ($(B)+(1,0)$) node {$t_2^-$};
\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$0^+$};



%\node[main1] (B1) at (B) {};
%\node[main1] (B2) at ($(B)-(0,0.5*\Ahgt)$) {};
%\draw[red,thick] (B1) -- (B2);

\node[main1] (i1) at ($(B)-(-0.15,-0.2*\Ahgt)$) {};
\node[main1] (i2) at ($(B)-(0.15,0.7*\Ahgt)$) {};
\draw ($(i1)+(0.25,0.1)$) node {\footnotesize $i_1$};
\draw ($(i2)+(0.28,0)$) node {\footnotesize $i_2$};
\draw[red,thick] (i1) -- (i2);

\node[main1] (A3) at ($(i)-(0,0.8*\Ahgt)+(-0.02,0.02)-(0,0.15)$) {};
\node[main1] (A4) at ($(A3)-(0.11,-0.15)$) {};
\node[main1] (A5) at ($(A3)+(0.11,-0.15)$) {};
\node[main2] (B3) at (C) {};
\node[main2] (B4) at ($(B3)-(0.2,0)$) {};
\node[main2] (B5) at ($(B3)+(0.2,0)$) {};
\foreach \n in {3,4,5}
{
\draw[red,thick] (i2) -- (A\n) -- (B\n);
}

\node [main1] (D1) at ($(A)+(0,-0.3)$) {};
\node [main1] (D2) at ($(A)+(0,-0.1)$) {};
\node [main1] (D3) at ($(A)+(0,0.1)$) {};
\node [main2] (E1) at ($(B)+(-0.2,-0.35)$) {};
\node [main2] (E2) at ($(B)+(-0.2,-0.2)$) {};
\node [main2] (E3) at ($(B)+(-0.2,-0.05)$) {};


\node [main2] (F1) at ($(A)+(0,0.7)$) {};
\node [main2] (F2) at ($(A)+(0,0.55)$) {};
\node [main2] (F3) at ($(A)+(0,0.4)$) {};
\node [main1] (G1) at ($(B)+(0,0.8)$) {};
\node [main1] (G2) at ($(B)+(0,0.6)$) {};
\node [main1] (G3) at ($(B)+(0,0.4)$) {};

\foreach \n in {1,2,3}
{
\draw [red,thick] (i2) -- (D\n) -- (E\n);
\draw [red,thick] (i1) -- (F\n) -- (G\n);
}
\end{tikzpicture}
\end{center}


==> figures/EM2b/aEM2b-2.tex <==
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=none,inner sep=1.5}, main2/.style = {circle,draw,fill=none,inner sep=2.25}]
\def\spacer{2};
\def\spacerr{1.5};
\def\Ahgt{1.2};
\def\Bhgt{1.2};

%\draw [fill=white,white] (0,1.35) circle [x radius=0.6cm,y radius=0.75cm];
%\draw [fill=white,white] (0,-1.45) circle [x radius=0.6cm,y radius=0.7cm];


\coordinate (B) at (\spacer,0);


\node[main1] (V1) at ($(-\spacerr,1.35)$) {};
\node[main1] (V2) at ($(-\spacerr,-0.1)$) {};
%\node[main1] (V3) at ($(-\spacerr,-1.45)$) {};

\node[main1] (A1) at (0,1.35) {};
\node[main1] (A2) at (0,-0.1) {};
%\node[main1] (A3) at (0,-1.45) {};
\foreach \n in {1,2}
{
\node[main1] (B\n) at ($(A\n)+(\spacer,0)$) {};
}



\foreach \n in {1,2}
{
\draw [thick,red] (V\n) -- (A\n) -- (B\n);
}
\draw [thick,red] (V1) -- (V2);

\draw ($(V1)-(0.5,0)$) node {$i_1$};
\draw ($(V2)-(0.5,0)$) node {$i_2$};
\foreach \where/\what in {A1/I_{1,1},B1/I_{1,2},A2/I_{2,1},B2/I_{2,2}}
{
\draw ($(\where)+(0,0.5)$) node {$\what$};
}


\draw ($(-\spacerr,0.625)-(1.8,0)$) node {$R_{\text{\bfseries EM2b}}':$};





%\draw (10.5,2) node {Type II};
\end{tikzpicture}


\begin{comment}
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=none,inner sep=1.5}, main2/.style = {circle,draw,fill=none,inner sep=2.25}]
\def\spacer{2};
\def\spacerr{1.5};
\def\Ahgt{1.2};
\def\Bhgt{1.2};

\draw [fill=white,white] (0,1.35) circle [x radius=0.6cm,y radius=0.75cm];
\draw [fill=white,white] (0,-1.45) circle [x radius=0.6cm,y radius=0.7cm];


\coordinate (B) at (\spacer,0);


\node[main1] (V1) at ($(-\spacerr,1.35)$) {};
\node[main1] (V2) at ($(-\spacerr,-0.1)$) {};
%\node[main1] (V3) at ($(-\spacerr,-1.45)$) {};

\node[main1] (A1) at (0,1.35) {};
\node[main1] (A2) at (0,-0.1) {};
\node[main1] (A3) at (0,-1.45) {};
\foreach \n in {1,2,3}
{
\node[main1] (B\n) at ($(A\n)+(\spacer,0)$) {};
}



\foreach \n in {1,2}
{
\draw [thick,red] (V\n) -- (A\n) -- (B\n);
}
\draw [thick,red] (V2) -- (A3) -- (B3);
\draw [thick,red] (V1) -- (V2);

\draw ($(V1)-(0.5,0)$) node {$i_1$};
\draw ($(V2)-(0.5,0)$) node {$i_2$};
\foreach \where/\what in {A1/I_{1,1},B1/I_{1,2},A2/I_{2,1},B2/I_{2,2},A3/I_{3,1},B3/I_{3,2}}
{
\draw ($(\where)+(0,0.5)$) node {$\what$};
}


\draw ($(V2)-(1.8,0)$) node {$R_{\text{\bfseries EM2b}}':$};





%\draw (10.5,2) node {Type II};
\end{tikzpicture}

\end{comment}

==> figures/EM2b/aEM2b.tex <==
\begin{center}
\begin{tikzpicture}[scale=.7,main/.style = {circle,draw,fill=none,inner sep=1}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0,-\Ahgt-2.5*\ver)$);

\draw[red,thick] ($(A)-(0.3,0)$) -- ($(C)-(0.3,0)$);
\draw[red,thick] ($(A)-(0.1,0)$) -- ($(C)-(0.1,0)$);
\draw[red,thick] ($(A)-(-0.1,0)$) -- ($(C)-(-0.1,0)$);
\draw[red,thick] ($(A)-(-0.3,0)$) -- ($(C)-(-0.3,0)$);

\draw[red,fill=red!60] ($(A)+(0,\Ahgt)$) -- ($(A)-(0,\Ahgt)$) -- ($(B)-(0,\Bhgt)$) -- ($(B)+(0,\Bhgt)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[fill=white] (A) circle [y radius=\Ahgt cm,x radius=0.6cm];
\draw[fill=white] (B) circle [y radius=\Bhgt cm,x radius=0.6cm];
\draw[fill=white] (C) circle [y radius=0.35 cm,x radius=0.35cm];

\draw ($(A)+(0,0)$) node {$I_A$};
\draw ($(B)+(0,0.5*\Ahgt)$) node {$I_B$};
\draw (C) node {$I_C$};
\draw ($(C)+(-1,0.85)$) node {$M$};

\draw ($(A)+(-0.75,1.75)$) node {$R_{\text{{\bfseries EM2b}}}:$};

\draw ($(A)+(-1,0)-(0.2,-0.2)$) node {$\geq t_2^+$};
\draw ($(B)+(1,0)+(0.2,-0.2)$) node {$\geq t_2^-$};
%\draw ($(A)+(-1,0)$) node {$t_2^+$};
%\draw ($(B)+(1,0)$) node {$t_2^-$};
\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$0^+$};



\node[main] (B1) at (B) {};
\node[main] (B2) at ($(B)-(0,0.5*\Ahgt)$) {};

\draw[red,thick] (B1) -- (B2);


\end{tikzpicture}
\end{center}


==> figures/EM2c/aEM2c-1.tex <==
\begin{center}
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=none,inner sep=1.2},main2/.style = {circle,draw,fill=none,inner sep=0.8}]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1.2};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0,-\Ahgt-2.5*\ver)$);
\coordinate (D) at ($(\spacer,-\Ahgt-2.5*\ver)$);


\draw[red,fill=red!20] ($(A)+(0,\Ahgt)$) -- ($(A)-(0,\Ahgt)$) -- ($(B)-(0,\Bhgt)$) -- ($(B)+(0,\Bhgt)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[fill=white,densely dotted] (A) circle [y radius=\Ahgt cm,x radius=0.6cm];
\draw[fill=white,densely dotted] (B) circle [y radius=\Bhgt cm,x radius=0.6cm];
\draw[fill=white,densely dotted] (C) circle [y radius=0.35 cm,x radius=0.35cm];
\draw[fill=white,densely dotted] (D) circle [y radius=0.35 cm,x radius=0.35cm];

%\draw ($(A)+(0,0.5*\Ahgt)-(0.5,0)$) node {$I_A$};
%\draw ($(B)+(0.5,0)$) node {$I_B$};
%\draw ($(C)+(0,0.5)$) node {$I_C$};


\draw ($(A)+(-1,0)$) node {$t_2^-$};
\draw ($(B)+(1,0)$) node {$t_1^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$0^{+}$};
\draw ($(D)+(1,0)$) node {$0^+$};

\node[main1] (i1) at ($(B)-(-0.15,0.4*\Ahgt)$) {};
\node[main1] (i2) at ($(A)-(0.1,0.3*\Ahgt)$) {};
\node[main2] (A3) at ($(A)-(0,0.6*\Ahgt)+(-0.02,0.02)-(0,0.2)$) {};
\node[main2] (A4) at ($(A3)-(0.11,-0.11)$) {};
\node[main2] (A5) at ($(A3)+(0.11,-0.11)$) {};
\node[main1] (B3) at (C) {};
\node[main1] (B4) at ($(B3)-(0.2,0)$) {};
\node[main1] (B5) at ($(B3)+(0.2,0)$) {};

\node[main1] (I3) at ($(B)-(-0.1,0.8*\Ahgt)+(-0.02,0.02)-(0,0.15)$) {};
\node[main1] (I4) at ($(I3)-(0.11,0.15)$) {};
\node[main1] (I5) at ($(I3)+(0.11,0.15)$) {};
\node[main2] (H3) at (D) {};
\node[main2] (H4) at ($(H3)-(0.2,0)$) {};
\node[main2] (H5) at ($(H3)+(0.2,0)$) {};

\node [main2] (D1) at ($(A)+(0.15,0.25)$) {};
\node [main2] (D2) at ($(A)+(0.15,0.05)$) {};
\node [main2] (D3) at ($(A)+(0.15,0.45)$) {};
\node [main2] (D4) at ($(A)+(0.15,0.65)$) {};
%\node [main1] (E1) at ($(B)-(0.1,0.1)+(0,0)$) {};
%\node [main1] (E2) at ($(B)-(0.1,0.1)+(0,-0.15)$) {};
%\node [main1] (E3) at ($(B)-(0.1,0.1)+(0,0.15)$) {};

%\node [main1] (F1) at ($(A)+(0.2,0.6)+(0,0)$) {};
%\node [main1] (F2) at ($(A)+(0.2,0.6)+(0,-0.15)$) {};
%\node [main1] (F3) at ($(A)+(0.2,0.6)+(0,0.15)$) {};
\node [main1] (G1) at ($(B)+(0,0.45)+(0,0)$) {};
\node [main1] (G2) at ($(B)+(0,0.45)+(0,-0.2)$) {};
\node [main1] (G3) at ($(B)+(0,0.45)+(0,0.2)$) {};
\node [main1] (G4) at ($(B)+(0,0.45)+(0,0.4)$) {};

\foreach \n in {1,2,3,4}
{
%\draw [red,thick] (i2) -- (E\n) -- (F\n);
\draw [red,thick] (i1) -- (D\n) -- (G\n);
}



\draw [red,thick] (i2) -- (i1);
\foreach \n in {3,4,5}
{
\draw[red,thick] (i1) -- (A\n) -- (B\n);
\draw[red,thick] (i2) -- (I\n) -- (H\n);
}



\draw ($(i2)+(-0.25,0.1)$) node {\footnotesize $i_2$};
\draw ($(i1)+(0.275,0.15)$) node {\footnotesize $i_1$};

\end{tikzpicture}
\end{center}


==> figures/EM2c/aEM2c-2.tex <==
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=none,inner sep=1.5}, main2/.style = {circle,draw,fill=none,inner sep=2.25}]
\def\spacer{2};
\def\spacerr{1.5};
\def\Ahgt{1.2};
\def\Bhgt{1.2};

%\draw [fill=white,white] (0,1.35) circle [x radius=0.6cm,y radius=0.75cm];
%\draw [fill=white,white] (0,-1.45) circle [x radius=0.6cm,y radius=0.7cm];


\coordinate (B) at (\spacer,0);


\node[main1] (V1) at ($(-\spacerr,1.35)$) {};
\node[main1] (V2) at ($(-\spacerr,-0.1)$) {};
%\node[main1] (V3) at ($(-\spacerr,-1.45)$) {};

\node[main1] (A1) at (0,1.35) {};
\node[main1] (A2) at (0,-0.1) {};
%\node[main1] (A3) at (0,-1.45) {};
\foreach \n in {1,2}
{
\node[main1] (B\n) at ($(A\n)+(\spacer,0)$) {};
}



\foreach \n in {1,2}
{
\draw [thick,red] (V\n) -- (A\n) -- (B\n);
}
\draw [thick,red] (V1) -- (V2);

\draw ($(V1)-(0.5,0)$) node {$i_1$};
\draw ($(V2)-(0.5,0)$) node {$i_2$};
\foreach \where/\what in {A1/I_{1,1},B1/I_{1,2},A2/I_{2,1},B2/I_{2,2}}
{
\draw ($(\where)+(0,0.5)$) node {$\what$};
}


\draw ($(-\spacerr,0.625)-(1.8,0)$) node {$R_{\text{\bfseries EM2c}}':$};





%\draw (10.5,2) node {Type II};
\end{tikzpicture}


==> figures/EM2c/aEM2c.tex <==
\begin{center}
\begin{tikzpicture}[scale=.7]
\def\spacer{2};
\def\Ahgt{1};
\def\Bhgt{1.2};
\def\ver{0.5};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0,-\Ahgt-2.5*\ver)$);
\coordinate (D) at ($(\spacer,-\Ahgt-2.5*\ver)$);

\draw[red,thick] ($(A)-(0.3,0)$) -- ($(C)-(0.3,0)$);
\draw[red,thick] ($(A)-(0.1,0)$) -- ($(C)-(0.1,0)$);
\draw[red,thick] ($(A)-(-0.1,0)$) -- ($(C)-(-0.1,0)$);
\draw[red,thick] ($(A)-(-0.3,0)$) -- ($(C)-(-0.3,0)$);

\draw[red,thick] ($(B)-(0.3,0)$) -- ($(D)-(0.3,0)$);
\draw[red,thick] ($(B)-(0.1,0)$) -- ($(D)-(0.1,0)$);
\draw[red,thick] ($(B)-(-0.1,0)$) -- ($(D)-(-0.1,0)$);
\draw[red,thick] ($(B)-(-0.3,0)$) -- ($(D)-(-0.3,0)$);

\draw[red,fill=red!60] ($(A)+(0,\Ahgt)$) -- ($(A)-(0,\Ahgt)$) -- ($(B)-(0,\Bhgt)$) -- ($(B)+(0,\Bhgt)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[fill=white] (A) circle [y radius=\Ahgt cm,x radius=0.6cm];
\draw[fill=white] (B) circle [y radius=\Bhgt cm,x radius=0.6cm];
\draw[fill=white] (C) circle [y radius=0.35 cm,x radius=0.35cm];
\draw[fill=white] (D) circle [y radius=0.35 cm,x radius=0.35cm];

\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw (C) node {$I_C$};
\draw (D) node {$I_D$};
\draw ($(C)+(-1,0.85)$) node {$M_1$};
\draw ($(D)+(1,0.85)$) node {$M_2$};

\draw ($(A)+(-0.75,1.75)$) node {$R_{\text{{\bfseries EM2c}}}:$};

%\draw ($(A)+(-1,0)-(0.2,0)$) node {$\geq t_2^-$};
%\draw ($(B)+(1,0)+(0.2,0)$) node {$\geq t_1^-$};
\draw ($(A)+(-1,0)$) node {$t_2^-$};
\draw ($(B)+(1,0)$) node {$t_1^-$};
%\draw ($(0.5*\spacer,1.5)$) node {$n^-$};
\draw ($(C)+(-1,0)$) node {$0^{+}$};
\draw ($(D)+(1,0)$) node {$0^+$};

%\draw[red,thick] ($(A)-(0,0*\Ahgt)$) -- ($(A)-(0,0.5*\Ahgt)$);



\end{tikzpicture}
\end{center}


==> figures/EM2d/aEM2d-1.tex <==
\begin{center}
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=white,inner sep=1.2},main2/.style = {circle,draw,fill=white,inner sep=0.8}]
\def\spacer{2};
\def\Ahgt{1.25};
\def\Bhgt{1.25};
\def\ver{0.3};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.5*\ver)$);

%\draw[red,thick] ($(A)-(0,0)$) -- ($(C)+(0,0.25)$) -- ($(B)-(0,0)$);
%\draw[red,thick] ($(A)-(0,0.25)$) -- ($(C)+(0,0)$) -- ($(B)-(0,0.25)$);
%\draw[red,thick] ($(A)-(0,0.5)$) -- ($(C)+(0,-0.25)$) -- ($(B)-(0,0.5)$);
%\draw[red,thick] ($(A)-(0,0.75)$) -- ($(C)+(0,-0.5)$) -- ($(B)-(0,0.75)$);
\draw[white,fill=white] ($(C)+(-0.5,-0.6)$) -- ($(C)+(0.5,-0.6)$) -- ($(C)+(0.5,-0.3)$) -- ($(C)+(-0.5,-0.3)$) -- cycle;

%\draw[red,fill=red!60] ($(A)+(0,\Ahgt)$) -- ($(A)-(0,\Ahgt)$) -- ($(B)-(0,\Bhgt)$) -- ($(B)+(0,\Bhgt)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[draw=red,densely dotted,fill=red!20] (A) circle [y radius=\Ahgt cm,x radius=0.6cm];
\draw[draw=red,densely dotted,fill=red!20] (B) circle [y radius=\Bhgt cm,x radius=0.6cm];
\draw[fill=white,densely dotted] (C) circle [y radius=0.5 cm,x radius=0.5cm];

%\draw ($(A)$) node {$I_A$};
%\draw ($(B)$) node {$I_B$};
%\draw (C) node {$I_C$};
%\draw ($(C)+(1.25,0.5)$) node {$M'$};
%\draw ($(C)+(-1.25,0.5)$) node {$M$};

\draw ($(A)+(-1,0)-(0.2,0)$) node {$\geq t_2^-$};
\draw ($(B)+(1,0)+(0.2,0)$) node {$\geq t_2^-$};
%\draw ($(A)+(-1,0)$) node {$t_2^+$};
%\draw ($(B)+(1,0)$) node {$t_2^+$};
\draw ($(0.5*\spacer,1.5)$) node {$n^-$};


\draw ($(C)+(0,-0.75)+(0.8,0.3)$) node {$0^+$};


\node[main1] (i1) at ($(A)-(0.25,0.7*\Ahgt)$) {};
\node[main1] (i2) at ($(C)-(0,0.3*\Ahgt)$) {};
\node[main1] (i3) at ($(B)+(0.25,-0.7*\Ahgt)$) {};

\node[main1] (A3) at ($(B)+(0.3,0.2)$) {};
\node[main1] (A4) at ($(A3)-(0,0.2)$) {};
\node[main1] (A5) at ($(A3)+(0,0.2)$) {};
\node[main1] (A6) at ($(A3)-(0,0.4)$) {};
\node[main2] (B3) at ($(B)+(-0.2,0.4)$) {};
\node[main2] (B4) at ($(B3)-(0.1,0.2)$) {};
\node[main2] (B5) at ($(B3)+(0.1,0.2)$) {};
\node[main2] (B6) at ($(B3)-(0.2,0.4)$) {};

\node[main1] (C3) at ($(A)+(-0.3,0.5)$) {};
\node[main1] (C4) at ($(C3)-(0,0.2)$) {};
\node[main1] (C5) at ($(C3)+(0,0.2)$) {};
\node[main1] (C6) at ($(C3)-(0,0.4)$) {};
\node[main2] (D3) at ($(A)+(0.2,0.7)$) {};
\node[main2] (D4) at ($(D3)-(-0.1,0.2)$) {};
\node[main2] (D5) at ($(D3)+(-0.1,0.2)$) {};
\node[main2] (D6) at ($(D3)-(-0.2,0.4)$) {};

\node[main2] (E1) at ($(A)+(0.35,-0.45)$) {};
\node[main2] (E2) at ($(E1)+(0.05,0.18)$) {};
\node[main1] (F1) at ($(C)+(0.2,0.1)$) {};
\node[main1] (F2) at ($(F1)+(0.05,0.18)$) {};

\node[main2] (G1) at ($(C)+(-0.15,0.05)$) {};
\node[main2] (G2) at ($(G1)+(0.1,0.15)$) {};
\node[main1] (H1) at ($(A)+(0.1,-0.9)$) {};
\node[main1] (H2) at ($(H1)+(0.1,0.15)$) {};

\draw ($(i2)-(0,0.35)$) node {\footnotesize $i_2$};
\draw ($(i1)-(0.3,0.15)$) node {\footnotesize $i_1$};
\draw ($(i3)+(0.3,-0.15)$) node {\footnotesize $i_3$};
\draw[red,thick] (i1) -- (i2) -- (i3);

\foreach \n in {3,4,5,6}
{
\draw[red,thick] (i3) -- (B\n) -- (A\n);
\draw[red,thick] (i1) -- (D\n) -- (C\n);
}

\foreach \n in {1,2}
{
\draw[red,thick] (i1) -- (E\n) -- (F\n);
\draw[red,thick] (i1) -- (G\n) -- (H\n);
}
\end{tikzpicture}
\end{center}


==> figures/EM2d/aEM2d-2.tex <==
\begin{tikzpicture}[scale=.7,main1/.style = {circle,draw,fill=none,inner sep=1.5}, main2/.style = {circle,draw,fill=none,inner sep=2.25}]
\def\spacer{2};
\def\spacerr{1.5};
\def\Ahgt{1.2};
\def\Bhgt{1.2};

\draw [fill=white,white] (0,1.35) circle [x radius=0.6cm,y radius=0.75cm];
\draw [fill=white,white] (0,-1.45) circle [x radius=0.6cm,y radius=0.7cm];


\coordinate (B) at (\spacer,0);


\node[main1] (V1) at ($(-\spacerr,1.35)$) {};
\node[main1] (V2) at ($(-\spacerr,-0.1)$) {};
\node[main1] (V3) at ($(-\spacerr,-1.45)$) {};

\node[main1] (A1) at (0,1.35) {};
%\node[main1] (A2) at (0,-0.1) {};
\node[main1] (A3) at (0,-1.45) {};
\foreach \n in {1,3}
{
\node[main1] (B\n) at ($(A\n)+(\spacer,0)$) {};
}



\foreach \n in {1,3}
{
\draw [thick,red] (V\n) -- (A\n) -- (B\n);
}

\draw [thick,red] (V1) -- (V2) -- (V3);

\draw ($(V1)-(0.5,0)$) node {$i_1$};
\draw ($(V2)-(0.5,0)$) node {$i_2$};
\draw ($(V3)-(0.5,0)$) node {$i_3$};
\foreach \where/\what in {A1/I_{1,1},B1/I_{1,2},A3/I_{3,1},B3/I_{3,2}}
{
\draw ($(\where)+(0,0.5)$) node {$\what$};
}


\draw ($(V2)-(1.8,0)$) node {$R_{\text{\bfseries EM2d}}':$};





%\draw (10.5,2) node {Type II};
\end{tikzpicture}


==> figures/EM2d/aEM2d.tex <==
\begin{center}
\begin{tikzpicture}[scale=.7]
\def\spacer{2};
\def\Ahgt{1.25};
\def\Bhgt{1.25};
\def\ver{0.3};
\def\wid{0.75};

\coordinate (A) at (0,0);
\coordinate (B) at (\spacer,0);
\coordinate (C) at ($(0.5*\spacer,-\Ahgt-2.5*\ver)$);

\draw[red,thick] ($(A)-(0,0)$) -- ($(C)+(0,0.25)$) -- ($(B)-(0,0)$);
\draw[red,thick] ($(A)-(0,0.25)$) -- ($(C)+(0,0)$) -- ($(B)-(0,0.25)$);
\draw[red,thick] ($(A)-(0,0.5)$) -- ($(C)+(0,-0.25)$) -- ($(B)-(0,0.5)$);
\draw[red,thick] ($(A)-(0,0.75)$) -- ($(C)+(0,-0.5)$) -- ($(B)-(0,0.75)$);
\draw[white,fill=white] ($(C)+(-0.5,-0.6)$) -- ($(C)+(0.5,-0.6)$) -- ($(C)+(0.5,-0.3)$) -- ($(C)+(-0.5,-0.3)$) -- cycle;

%\draw[red,fill=red!60] ($(A)+(0,\Ahgt)$) -- ($(A)-(0,\Ahgt)$) -- ($(B)-(0,\Bhgt)$) -- ($(B)+(0,\Bhgt)$) -- cycle;
%\draw[red,fill=red!60] (C) -- ($(A)+(0,-\Ahgt)$) -- ($(A)+(\wid,0)+(-0.3,0.9)$) -- (C);
%\draw[red,fill=red!60] (C) -- ($(B)-(\wid,0)-(-0.3,-0.9)$) -- ($(B)+(0,-\Bhgt)$) -- cycle;


\draw[fill=red!60] (A) circle [y radius=\Ahgt cm,x radius=0.6cm];
\draw[fill=red!60] (B) circle [y radius=\Bhgt cm,x radius=0.6cm];
\draw[fill=white] (C) circle [y radius=0.5 cm,x radius=0.5cm];

\draw ($(A)$) node {$I_A$};
\draw ($(B)$) node {$I_B$};
\draw (C) node {$I_C$};
\draw ($(C)+(1,0.4)$) node {$M'$};
\draw ($(C)+(-1,0.4)$) node {$M$};

\draw ($(A)+(-0.75,1.75)$) node {$R_{\text{{\bfseries EM2d}}}:$};

\draw ($(A)+(-1,0)-(0.2,0)$) node {$\geq t_2^-$};
\draw ($(B)+(1,0)+(0.2,0)$) node {$\geq t_2^-$};
%\draw ($(A)+(-1,0)$) node {$t_2^+$};
%\draw ($(B)+(1,0)$) node {$t_2^+$};
\draw ($(0.5*\spacer,1.5)$) node {$n^-$};


\draw ($(C)+(0,-0.75)+(0.8,0.3)$) node {$0^+$};



\end{tikzpicture}
\end{center}

